LSIAC-MRA for Nonuniform Meshes and Applications to Mesh Adaptivity

In this article we consider the extension of the (L)SIAC-MRA enhancement procedure to nonuniform meshes. We demonstrate that error reduction can be obtained on perturbed quadrilateral and Delaunay meshes, and investigate the effect of limited resolution and its impact on the procedure for various function types. We show that utilizing mesh-based localized kernel scalings, which were shown to reduce approximation errors for LSIAC filters, improve the performance of the LSIAC-MRA enhancement procedure. Lastly, we demonstrate the usefulness of enhanced approximations generated by (L)SIAC-MRA in mesh adaptivity applications, and show that SIAC reconstruction can be used in identification of regions of high error in steady-state DG approximations.

==> adaptive_scaling.tex <==

\section*{Adaptive kernel scaling}

Here an adaptive kernel scaling given by Jallepalli is used.  This consists of a preprocessing step to assigning a characteristic length to each vertex in the mesh, and then a postprocessing step where based off the location of the filtering point in an element, a weighting of the characteristic lengths of the vertices in that element produces a characteristic length. 
Let $v_i$ be the $i$-th vertex in the mesh, $e_j$ an element with vertex $v_i$, and $L_{e_j}$ the length of the edge of $e_j$ with maximum length. Then we assign a characteristic length $H$ to vertex $v_i$ via the expression:

\[
H(v_i)=\frac{\sum_{j}L_{e_j}\cdot Area(e_j)}{\sum_{j}Area(e_j)}.
\]
Then given a filtering point $x^{\star}$, we compute the characteristic scaling via the relation
\[
H(x^{\star})=\sum_{\ell=0}^N\lambda_{\ell}H(v_{\ell})
\]
where $v_{\ell}$ are the vertices of the element containing $x^{\star}$ and $\lambda_{\ell}$ are the barycentric coordinates of $x^{\star}$ in that element.

\subsection{Adaptive scaling on a 1D mesh}
On a 1D mesh with $I_j=[x_{j-1/2},x_{j+1/2}]$ and $\Delta x_j=x_{j+1/2}-x_{j-1/2}$ for $j=1:N$, we have
\begin{align*}
    H(x_{1/2})&=\Delta x_1,\\
     H(x_{j-1/2})&=\frac{(\Delta x_{j})^2+(\Delta x_{j-1})^2}{\Delta x_{j}+\Delta x_{j-1}},\text{ for } j=2:N,\\
      H(x_{N+1/2})&=\Delta x_N.
\end{align*}
Supposing the filtering point $x^{\star}$ is in element $I_j$, we then have the characteristic scaling:

\begin{align*}
    H(x^{\star})&=\xi_j H(x_{j-1/2})+(1-\xi_j)H(x_{j+1/2}),
    \intertext{where}
    \xi_j&=\frac{1}{\Delta x_j}(x-x_{j-1/2})
\end{align*}


==> sections/mesh_gen_and_refinement.tex <==

\section{Meshes Generation and Refinement}\label{sec:mesh}
In this section we describe the mesh generation and refinement procedure employed in this work and provide several examples of different meshes generated by this technique. The following procedure generates nonuniform, but conforming (no hanging nodes) meshes. 
\subsection{Nonuniformity by Node Perturbation}
Starting with a set of nodes $\{\mathbf{v}_i\}_{i=1}^{\#_{nodes}}$ $\mathbf{v}_i\in \mathbf{R}^d$ ($d=1,2$), which defines an associated uniform mesh over the domain $\Omega$, we perturb each interior node,
\[\mathbf{\tilde{v}}_i=\mathbf{v}_i+\epsilon_i\] 
where  $\epsilon_i$ is a random quantity. Specifically we consider
\[\epsilon_i=\mathbf{p}.*\mathbf{u}\]
where $\mathbf{u}$ is a vector whose entries are sampled from a uniform distribution over $[-1/2,1/2]$, $\mathbf{p}$ is a vector of non-negative numbers scaling the maximum perturbation possible, and $.*$ represents an element-wise multiplication. Here we require the entries of $\mathbf{p}$ be smaller than one to prevent a possible crossing or fusing of nodes. 

Since we are considering a periodic rectangular domain in this work, we do not apply the perturbation in a given direction to boundary nodes if it would move that node off the boundary. Furthermore, to maintain the periodic conforming nature of the mesh, we use the same perturbation for nodes that are periodically associated on the boundaries.  Having obtained our set of perturbed nodes $\{\mathbf{\tilde{v}}_i\}\}_{i=1}^{\#_{nodes}}$ we now define the nonuniform mesh. In one dimension, or in the quadrilateral case, we simply use the same elements as in the uniform case, but now instead use the perturbed nodes to generate the nonuniformity. In the triangular case, we define the mesh via a Delaunay triangulation of the perturbed nodes. Examples of meshes resulting from this procedure are provided in Figure \ref{fig:mesh_examples}.

\input{Figures/meshes/mesh_examples.tex}

\subsection{Meshes with greater variability in element sizes}

For the purposes of consider the effects of adaptive scaling on the enhanced reconstruction procedure, we also consider the following three meshes (depicted in Figure \ref{fig:adaptive_mesh_examples}) generated by using the GMSH application \cite{gmsh}. We denote these meshes as SVR10, SVR100, and ISR2. Here SVR10 (SVR100) denotes a smoothly varying mesh where the ratio of the boundary to center element is 10 (100), while ISR2 denotes a mesh with a more abrupt transition between boundary elements and interior elements with an element size ratio of 2.

\input{Figures/adap_scaling/adaptive_mesh_examples}

\subsection{Mesh Refinement}
For refinement we consider a uniform subdivision into $2^d$ elements. In two dimensions there are multiple ways do this so we describe our approach. Here our subdivision is interpolary in that nodes on the coarse mesh remain present after refinement. The procedure is as follows for every edge on the mesh insert a node at the midpoint of that edge (in the quadrilateral case we also insert a node at the average of the midpoints of the edges of each element). We then connect these new nodes with the original nodes to form four new elements on the refined mesh. A depiction of this subdivision procedure is shown in Figure \ref{fig:subdivision}.
\input{Figures/meshes/subdivision.tex}
